Top Score in Axelrod Tournament

The focus of the project will be an examination of obtaining the highest score in the Axelrod Tournament. The initial design of the highest score in the Axelrod Tournament consisted of looking at the Cooperation rates of the top strategies currently in the Axelrod Library. After creating an initial Finite State Machine strategy that utilized the Cooperation Rates of the top players; our ten-state FSM finished within the top 35 players out of 220 in the short run time strategies in the Axelrod Library. After a quick evolutionary algorithm, 50 generations, our original ten-state FSM was changed into an eight-state FSM, which finished within the top 5 of the short run time strategies in the Axelrod Library. This eight-state FSM was then evolved again using a full evolutionary algortihm process, which lasted 500 generations, where the eight-state FSM evolved into a another eight-state FSM which finishes first in the Axelrod Library among the short run time strategies and the full Axelrod Tournament. From that final FSM, two of the eight states are inaccessible, so the final FSM strategy is a six-state FSM that finishes first in the Full Axelrod Tournament, against the short run time strategies as well as the long run time strategies.

==> TIKZ_Practice/profdiagramtext.tex <==
Going from the 8-state FSM diagram to a 6-state diagram:\\
Start at State 5. State 5 has two possibilities, stay in State 5 or go to State 7. There are now possible two states in the FSM. From State 7, there are two possibilities, go to State 4 or go to State 6, which leaves us with four states. The two possibilities from State 4 are to go to State 5 or go back to State 7. These are two previous states that have been identified. There are still four states. From State 6, there are two possibilities, go to State 3 or to State 8. Now there are six possible states. The possibilities for State 3 are to stay in State 3 or go to State 8. Those two possibilities are already in the FSM, so there are no new states being created. State 8 will either go to State 3 or will go back to State 4, and both of these states have been identified. This shows that there is no need to go be in State 1 or State 2 because that will never occur in this FSM since our initial state is State 5. So the 8-state FSM can be rewritten as a 6-state FSM.

\begin{center}

Transition States:\\
$(1, C, 3, C)$,
$(1, D, 8, C)$,\\
$(2, C, 1, D)$,
$(2, D, 5, D)$,\\
$(3, C, 3, D)$,
$(3, D, 8, D)$,\\
$(4, C, 7, D)$,
$(4, D, 5, C)$,\\
$(5, C, 5, C)$,
$(5, D, 7, D)$,\\
$(6, C, 3, D)$,
$(6, D, 8, D)$,\\
$(7, C, 4, C)$,
$(7, D, 6, D)$,\\
$(8, C, 3, C)$,
$(8, D, 4, D)$
\end{center}
